Impact of Large Language Model Assistance on Patients Reading Clinical Notes: A Mixed-Methods Study

Large language models (LLMs) have immense potential to make information more accessible, particularly in medicine, where complex medical jargon can hinder patient comprehension of clinical notes. We developed a patient-facing tool using LLMs to make clinical notes more readable by simplifying, extracting information from, and adding context to the notes. We piloted the tool with clinical notes donated by patients with a history of breast cancer and synthetic notes from a clinician. Participants (N=200, healthy, female-identifying patients) were randomly assigned three clinical notes in our tool with varying levels of augmentations and answered quantitative and qualitative questions evaluating their understanding of follow-up actions. Augmentations significantly increased their quantitative understanding scores. In-depth interviews were conducted with participants (N=7, patients with a history of breast cancer), revealing both positive sentiments about the augmentations and concerns about AI. We also performed a qualitative clinician-driven analysis of the model's error modes.

==> files/key_points.tex <==
\section*{1-2 Sentence Summary}%\label{sec:key_points}
In a mixed-methods investigation including a randomized survey with 200 participants and qualitative interviews with seven patients who previously had breast cancer, we found that large language model-based augmentations enhance the patient experience of reading clinical oncology notes. Furthermore, we found that careful validation of augmentations was required to avoid introducing harmful errors.



==> old_abstract.tex <==
\begin{comment}
 Patients derive numerous benefits from reading their clinical notes, including an increased sense of control over their health and improved understanding of their care plan. However, complex medical concepts and jargon, especially in the field of oncology, can hinder patient comprehension.
We leverage large language models (LLMs) to develop a patient-facing tool that makes clinical notes more readable. We prompt engineered GPT-4 to perform augmentations including simplifying, extracting information from, and adding context to the notes. We piloted the tool using clinical notes donated by breast cancer survivors and synthetic notes generated by a clinician. Augmentations were evaluated for errors by clinicians.
A set of female-identifying, US-based participants (N=200) were randomly assigned three clinical notes in our tool, with varying levels of augmentations.
After interacting with each note, patients answered questions evaluating their understanding of follow-up actions. 
In-depth interviews of self-identifying breast cancer patients (N=7) were also conducted.
Augmentations were associated with a significant increase in action understanding score (0.63 +/- 0.04 for select augmentations, compared to 0.54 +/- 0.02 for the control) with $p=0.002$. 
With augmentations, participants improved in score and confidence for real donated notes compared to synthetic notes.  Participants expressed positive sentiment about all augmentations. Participants preferred the augmentation that defined medical terminology in the note. Some participants voiced concern about relying on artificial intelligence. Clinicians identified minor misleading errors in the augmentations. Errors were more commonly found in augmented real notes than in synthetic notes. Augmentations improved some but not all readability metrics. 
This work demonstrates the potential of LLMs to improve cancer patients' experiences with clinical notes at a low burden to clinicians.
\end{comment}

==> old_intro.tex <==
\section*{Introduction}\label{ch:introduction}

The rapid advancement and improved performance of natural language processing could reduce barriers in communication and make information accessible to wider populations. Language models have the potential to help personalize and tailor the level and format of messaging to a variety of needs, e.g. to facilitate new avenues for public interest communication. Medicine, and public health more broadly, could particularly stand to benefit from new innovations in this space to facilitate improved patient-provider interaction. 

The information needs of patients are not well addressed by existing clinical workflows. Appointments are often too short to go fully in depth, and patients forget x\% of information conveyed during clinical visits [TODO cite]. % Clinicians have been found to frequently use unexplained medical jargon in appointments with patients \cite{MILLER20221261}, 
% and patients have been shown to misunderstand these terms
% \cite{10.1001/jamanetworkopen.2022.42972, SCHNITZLER2017112}.
% This shows that healthcare is a context where personalized communication could have high impact.
In response, patients' rights advocates pushed for increased transparency by enabling patients to read and access their own clinical notes, which generally function as physician-authored summaries of an encounter.  Reviewing clinical notes after an appointment can enable patients to better understand their medical conditions and improve care plan adherence [TODO cite]. In 2021, the $\textrm{21}^{st}$ Century Cares Act was expanded to mandate providers to make clinical notes digitally available to all patients \cite{blease2020opennotes, salmi2020clinicianviews}. 

 
Unfortunately, the clinical notes in electronic health records are written for the audiences of the clinician themselves, other clinicians involved in care, and administrative/billing users\cite{davidson2004s}. As a result, patients themselves are not the intended audience, and the medical jargon in clinical notes can be prohibitively difficult to understand. A recent study found it was the most frequently reported barrier to reading clinical notes \cite{kambhamettu2024explainable}. 
 







% In recent years, clinical notes have been an increasingly popular format of text-based communication between clinicians and patients \cite{Johnson}.
% Clinical notes are traditionally written by clinicians throughout a patient's treatment as a form of record-keeping.
% The notes are useful to doctors for keeping track of a patient's medical history and treatment \cite{papyrus_gillum}.
% The notes are also useful for patients to keep track of information from their appointments (a detailed discussion can be found in Section \ref{sec:notes_benefits}).
As a result, there have been efforts to cater clinical note-writing to patients.
However, medical professionals already experience an increased workload due to the adoption of electronic health record technology, which increases time spent on clinical review and documentation \cite{carayon, Gardner}, and report burnout \cite{10.1001/jama.2018.12777}.
The process of writing patient-facing notes puts an additional burden on clinicians, as it increases time spent on documentation \cite{10.1001/jama.2018.12777}. 

Artificial intelligence offers opportunities to enhance clinical note readability both during the clinician's process writing the note and the patient's experience reading the note. 
Prior research has explored AI-powered tools that assist clinicians during note composition, incorporating autocomplete features to facilitate structured data extraction and promote consistent, patient-friendly language \cite{murray2021medknowts, van2020automets}.



%Language modeling provides an opportunity to close the knowledge gap between clinicians and patients without introducing an additional burden on overworked clinicians.

In this paper, we take a patient-centric approach, and propose a set of augmentations that can be implemented using modern language modeling technology and applied to clinical notes to improve their readability for patients. We focus on breast cancer patients, as it is a chronic disease, resulting in an extensive series of clinical notes due to the multitude of appointments involved in treatment. 
We propose an implementation and user-centric interface (see Figure \ref{fig:intro-ui}) for these augmentations and evaluate them with a mixed methods approach, including interviews with breast cancer patients and user studies.

\begin{figure}
    \centering
    \includegraphics[width=16.5cm]{images/full_user_interface.png}
    \caption{
    Our proposed user interface for augmented clinical notes.
    \textbf{(A)} The user is able to switch between their original note and a simplified version using tabs.
    \textbf{(B)} The user's note (either the original or simplified depending on the selected option) is displayed with clear formatting.
    \textbf{(C)} Medical terms are highlighted in bold green and underlined to indicate that the user is able to click on them.
    When a user clicks on a medical term, the page will automatically scroll to the corresponding definition in \textit{(G)}
    \textbf{(D)} A title briefly describes the content of the clinical note.
    \textbf{(E)} Users can explore a series of questions designed to enhance their understanding of the note. 
    By clicking on a question, its corresponding answer will be revealed.
    \textbf{(F)} Tabs enable seamless navigation between different augmentations, providing a convenient way to switch between them. 
    The figure does not depict the \textit{Key Info} and \textit{To-Do List} augmentations, which display medication and appointment data as well as action items, respectively.
    \textbf{(G)} A scrollable sidebar is utilized to present definitions of medical terms.
    \textbf{(H)} An options menu allows the user to toggle the augmentations they wish to enable for their note.
    }
    \label{fig:intro-ui}
\end{figure}

% \subsection*{Scope}
% This work serves as a step towards automating personalized health communication, aiming to alleviate the burdens of medical communication for both patients and clinicians.
% Ultimately, our goal is to contribute towards the development of a publicly accessible tool that empowers patients to navigate their clinical notes more effectively. 

% This paper focuses on the development of a comprehensive set of augmentations, encompassing language simplification, information and context enhancement, and valuable information extraction, with the aim of enhancing the overall accessibility of clinical notes. 
% By choosing from this suite of augmentations, patients will have the ability to swiftly and effortlessly retrieve the necessary information to enrich their individual reading experience.

% Our research focuses exclusively on clinical notes pertaining to breast cancer patients, as this narrower scope allows us to gather specialized data and simplifies tasks by confining them to a specific domain rather than requiring generalization across all diseases and health emergencies. 
% %Furthermore, the breast cancer community typically exhibits a high level of engagement in research, as many survivors actively contribute to alleviating the burden on future patients, allowing us to recruit breast cancer survivors for user testing.
% Additionally, breast cancer is a chronic disease, resulting in an extensive series of clinical notes due to the multitude of appointments involved in treatment. 
% These clinical notes hold immense value for breast cancer patients, aiding them in managing the complexities of their treatment process. 
% Consequently, our tool aims to enhance patient understanding, facilitating informed decision-making and instilling confidence in treatment outcomes, by providing easier navigation of information from their appointments.

% \subsection*{Organization}
% % organization.
% We will begin by reviewing the current state of clinical notes and the \textit{Open Notes} movement in Chapter \ref{ch:opennotes}.
% This includes background information the health impacts of making clinical notes available to patients and how these impacts relate specifically to cancer treatment. 
% Chapter \ref{ch:modifications} identifies various categories of augmentations that can be implemented in clinical notes. Additionally, this chapter reviews prior studies and research involving the application of natural language processing techniques to realize these augmentations.
% In Chapter \ref{ch:implementations}, we present our own implementations of these augmentations.
% To evaluate the impact of the proposed augmentations on breast cancer notes, Chapter \ref{ch:evaluations} presents a comprehensive analysis of a quantitative user study, and Chapter \ref{sec:study2} presents the results of a qualitative study with former breast cancer patients to ascertain the extent of the augmentations' value.
% Finally, in Chapter \ref{ch:conclusion} we reflect on the findings of our work and discuss avenues for future explorations on AI augmentations for clinical notes.

% \section*{Background on Open Clinical Notes}\label{ch:opennotes}
% Clinical notes were  traditionally written for the sole purpose of physicians' records, and their contents were not shared with patients. 
% Since their inception, access to these notes and the format of them has slowly evolved. 
% These notes were standardized as medical records in the early 20th century to facilitate collaboration between clinicians caring for a single patient \cite{papyrus_gillum}. 

% In the late 20th century, patients' rights advocacy pushed for transparency in medical practices. 
% Several factors, such as the adoption of patients' rights bills by hospitals, the emergence of electronic health records, and \textit{The Health Insurance Portability and Accountability Act} (HIPPA) in 1996, made personal medical information, such as test results, medical images, and clinical notes, available to patients \cite{OpenNotes_history}. 
% Patient portals were introduced shortly after, allowing patients easier access to some of their medical records.
% During this time, clinical notes were not commonly available for patients to read online \cite{OpenNotes_history}.

% Clinical notes started becoming available for patients due to the \textit{OpenNotes} \cite{OpenNotes_website} organization, founded at the Beth Israel Deaconess Medical Center in Boston, which advocated for clinical notes describing patient visits to be shared with patients starting in 2010.
% In 2012, the group began running studies with their patients to validate the positive health impacts of giving patients digital access to their medical records (known as Electronic Health Records,  or \textit{EHRs}) \cite{delbanco}.
% These health benefits will be detailed in Section \ref{sec:notes_benefits}.

% Because of these benefits, hospitals began making clinical notes increasingly available in patient portals.
% The increased access to electronic health records has coincided with a rise in patient portal usage from 25\% of Americans accessing their patient portal in 2014 to 38\% in 2020 \cite{Johnson}.
% In 2021, the $\textrm{21}^{st}$ Century Cares Act was expanded to mandate providers to make clinical notes digitally available to all patients, including cancer patients, who had previously often had notes withheld \cite{blease2020opennotes, salmi2020clinicianviews}.


% \section*{Benefits of Open Note Policies}\label{sec:notes_benefits}

% Adopting open note policies has been linked to several benefits for patients such as self-reported health benefits and engagement, identifying treatment errors and inconsistencies, and making more information available to care partners.

% First, the original OpenNotes study showed that giving patients access to their clinical notes led to several self-reported benefits.
% Patients who read their clinical notes reported a higher sense of control of their care, a better understanding of their condition, and a stronger recollection of their care plan \cite{delbanco}.
% Up to 87\% of patients who accessed their medical records reported an increased sense of control over their health, and patients who read four or more clinical notes in the past twelve months scored significantly higher on a measure of shared decision-making with their provider \cite{delbanco}.
% Additionally, 92\% of patients better remember their plan for care \cite{nazi2014va}, 89\% better prepared for visits \cite{nazi2014va}, and 
% 80\% experienced improved medication adherence \cite{nazi2014va, desroches2019managing}. These trends continued to be observed in a follow-up study conducted seven years later \cite{walker2019seven_years}.


% Another benefit of Open Notes is that allowing patients to access their notes has helped make both parties more accountable, catching more mistakes in their medical records and improving adherence to plans. 
% Providers are held accountable because patients can review their clinician's understanding of their symptoms and medical history, helping them to identify misunderstandings \cite{Esch}, as errors in electronic health records are common \cite{kaboli,yadav}, with 21\% of patients who had read their clinical notes in the last year reporting a perceived mistake \cite{Bell}.
% In fact, about a third of patients who read their notes do so to look for errors in their notes \cite{Bell262}.
% Open notes support patients in finding  these errors that a clinician might miss. 
% Furthermore, patients are held accountable because they have a record of action items resulting from their appointments.
% This has been shown to make them more likely to take medication as prescribed and to follow through on recommended lifestyle changes
% \cite{Esch, delbanco, desroches2019managing}.


% Finally, vulnerable patients often rely on family members and friends as care partners \cite{LAIDSAARPOWELL20133, WOLFF2011823}, and open note policies may be beneficial because they improve the availability of information to care partners, even when care partners may not be available during an appointment \cite{wolff2016inviting}. 
% According to a study by Jackson et al. \cite{JACKSON2022290}, care partners reported numerous benefits when accessing clinical notes, including assistance in remembering the care plan, facilitating coordination with clinicians, and reducing the stress associated with caregiving. 
% The study also revealed that care partners consistently held more positive opinions regarding the significance of accessing clinical notes compared to patients.
% Another study \cite{wolff2016inviting} showed that care patients were more likely to access clinical notes and reported benefits to coordinating with clinicians.


% \subsection*{Remaining Issues With Open Notes}\label{sec:on-issues}
% Although sharing electronic health records with patients has been shown to yield numerous health benefits, there remains a need for improvement in the note-reading process. 
% Research indicates that a subset of patients, ranging from 3\% to 8\%, found reading their clinical notes to be more confusing than helpful \cite{delbanco}. 
% These patients are typically older, less educated, and in poorer health conditions \cite{root2016characteristics}. 
% One major challenge reported by patients is the difficulty in understanding medical terminology \cite{kujala2022experiences, kayastha}. 

% The open note policies have significantly changed the style in which notes are written to try to address these issues \cite{rahimian,rahimian2019significant}.
% Clinicians are now trained to write notes with their patients in mind, which involves including explanations and writing at a lower grade level, leading to more time spent on documentation \cite{desroches}.
% However, this may be an unreliable solution as clinicians are experiencing increased burnout due to the adoption of electronic health records \cite{carayon, Gardner}.

% The importance placed on writing patient-readable notes may not be uniformly prioritized among clinicians, as a considerable portion of them consistently exhibit greater skepticism towards the benefits of open notes compared to patients and perceive them as less significant \cite{delbanco, salmi2020clinicianviews}. This discrepancy in perspectives suggests that not all clinicians prioritize the optimization of notes for patient comprehension.

% \subsection*{Open Notes and Breast Cancer}\label{sec:notes_benefits_cancer}
% Enabling breast cancer patients to access their clinical notes presents both advantages and challenges. 
% The process of breast cancer treatment is known to be highly distressing and overwhelming, thereby necessitating that patients' specific and essential needs are met when engaging with their clinical notes \cite{cancer_notes}.


% Several of the benefits from Open Notes in general, such as self-reported health benefits and engagement, identifying treatment errors and inconsistencies, and making more information available to care partners, are especially true for breast cancer patients. 
% Breast cancer patients can face a greater information burden than other patients due to the number of encounters,  complex treatment, and sometimes counterintuitive terms, such as the dangerous, but seemingly harmless, \textit{triple negative} breast cancer \cite{salmi2020clinicianviews}. 
% With access to notes, patients reported increased comprehension, relieved anxiety, and increased trust \cite{kayastha}. 
% These findings were supported by another study, in which 96\% of patients reported improved understanding of their diagnosis, 94\% reported better understanding of treatment side effects, and 96\% reported feeling more reassured about their treatment \cite{SHAVERDIAN2019102}. 
% Furthermore, patients reporting poor health were more likely to report that notes weren't accurate or were missing important information \cite{Leveille2020evaluate}.
% Finally, for breast cancer patients, care partners are especially important, not only because the material is complicated, but also because cancer treatment (such as chemotherapy) is known to cause brain fog and make the treatment plan more difficult to navigate.
% Because of these benefits, patients overwhelmingly support access to clinical notes, with 98\% of cancer patients in favor \cite{salmi2020clinicianviews}. 
% Oncologists and physicians are generally supportive as well, with 73\% of physicians at a university in Sweden believing access to oncology notes is a good idea  \cite{blease2020opennotes}, and 78\% of oncologists supporting open note policies for cancer treatment \cite{salmi2020clinicianviews}.

% However, there are also some concerns that arise in the context of breast cancer in particular. 
% One study found that 44\% of clinicians believed cancer patients would experience confusion when reviewing their notes, whereas only 4\% of patients reported actual confusion \cite{salmi2020clinicianviews}. 
% Nonetheless, it is important to acknowledge that even though the percentage is relatively low, it still represents a significant number of patients who may encounter confusion when interacting with their clinical notes.
% While some clinicians are taking more time to write notes in the presence of open notes policies to help mitigate this concern, including 58\% of physicians at a university in Sweden  \cite{blease2020opennotes}, oncologists report concerns over altering the style and content of their note, fearing that it might compromise the integrity of their notes \cite{Alpert}. 
% This is likely a more serious concern with cancer patients as opposed to the general population, as studies have shown few patients report increased levels of worry after reading their clinical notes \cite{walker2019seven_years, desroches2019managing}, while about a quarter of cancer patients report feeling increased feelings of anxiety when reading their notes in qualitative interviews \cite{kayastha}. 





% \subsection*{Opportunities for Artificial Intelligence to Improve Clinical Notes}\label{sec:notes_needs}


% This paper will focus on the patient's perspective reading their notes, investigating how clinical notes can be modified to improve the reading experience. 
% By exploring augmentations that can be implemented in the patient's portal, this research aims to enhance the accessibility and comprehension of clinical notes, leveraging AI techniques to simplify language, provide context, and improve overall readability.
% A benefit of tackling the problem from the patient's perspective is that clinicians do not have to alter their initial notes, which clinicians report hesitation for as it might compromise the quality and integrity of their notes \cite{Alpert}.
% The motivation stems from the recognition that each patient has unique needs, abilities, and preferences when it comes to interacting with their healthcare.
% Even if clinicians are proficient at writing clear and comprehensive notes, it is essential to address the individualized nature of patient engagement.
% Our primary objective is to remove the barriers that hinder individuals from comprehending medical notes, making the information more accessible and understandable. Additionally, we aim to enhance the reading experience for all patients, regardless of their initial level of comfort with clinical notes.

